Improving Social Meaning Detection with Pragmatic Masking and Surrogate Fine-Tuning

Masked language models (MLMs) are pre-trained with a denoising objective that is in a mismatch with the objective of downstream fine-tuning. We propose pragmatic masking and surrogate fine-tuning as two complementing strategies that exploit social cues to drive pre-trained representations toward a broad set of concepts useful for a wide class of social meaning tasks. We test our models on $15$ different Twitter datasets for social meaning detection. Our methods achieve $2.34\%$ $F_1$ over a competitive baseline, while outperforming domain-specific language models pre-trained on large datasets. Our methods also excel in few-shot learning: with only $5\%$ of training data (severely few-shot), our methods enable an impressive $68.54\%$ average $F_1$. The methods are also language agnostic, as we show in a zero-shot setting involving six datasets from three different languages.

==> t5_para.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Praphrase Model}\label{sec:para} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In order to paraphrase our datasets, we fine-tune the T5\textsubscript{BASE} model~\cite{raffel2020exploring} on $4$ paraphrase datasets from PIT-2015 (tweet)~\cite{xu2015semeval},  {LanguageNet} (tweet)~\cite{lan2017continuously}, {Opusparcus} ~\cite{creutz2018open}  (video subtitle), and Quora Question Pairs (Q\&A website) \footnote{\url{https://www.quora.com/q/quoradata/First-Quora-Dataset-Release-Question-Pairs}}. For PIT-2015, LanguageNet and Opusparcus, we only keep sentence pairs with a semantic similarity score $\geq 70\%$. We then merge all datasets and shuffle them. Next, we split the data into Train, Dev, and Test ($80\%$, $10\%$, and $10\%$) and fine-tune T5 on the Train split for $20$ epochs with constant learning rate of $3e-4$. 

==> table/full_res.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{sidewaystable}
\centering
% \begin{table}
\tiny
\centering
\begin{tabular}{@{}lccccccccccccccccccc@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Task}}} & \multirow{2}{*}{\textbf{RoBERTa}} & \multirow{2}{*}{\textbf{RM-NR}} & \multirow{2}{*}{\textbf{BERTweet}} & \multicolumn{10}{c}{\textbf{PMLM}}                                                                                                                                     & \multicolumn{4}{c}{\textbf{SFT}}                                        & \multicolumn{2}{c}{\textbf{MT}}      \\ \cmidrule(lr){5-14} \cmidrule(lr){15-18} \cmidrule(lr){19-20} 
\multicolumn{1}{c}{}           &                    &                                   &                                    & \textbf{RM-N} & \textbf{PM-N}  & \textbf{RM-HA} & \textbf{PM-HA} & \textbf{RM-HE} & \textbf{PM-HE} & \textbf{RM-EA} & \textbf{PM-EA} & \textbf{RM-EE} & \textbf{PM-EE} & \textbf{SFT-E} & \textbf{X1+SFT-E} & \textbf{SFT-H} & \textbf{X2+SFT-H} & \textbf{RoBERTa} & \textbf{X2+SFT-H} \\ \midrule
Crisis\textsubscript{Oltea-14}    & 95.95   &       95.78                    & 95.88                              & 95.78         & 95.92          & 95.75          & 95.85          & 95.85          & 95.87          & 95.91          & 95.98          & 95.95          & 95.77          & 95.76          & \textbf{96.02}    & 95.87          & 95.68             & 95.88            & 95.70             \\
Emo\textsubscript{Moham-18}       & 77.99        &  79.15                     & 80.14                              & 79.43         & 80.73          & 80.31          & 78.56          & 79.51          & 80.15          & 80.03          & 81.09          & 81.28          & \textbf{82.18} & 79.69          & 82.04             & 78.69          & 80.50             & 75.79            & 75.85             \\
Hate\textsubscript{Waseem-16}     & 57.34          &  57.22                   & 57.47                              & 56.75         & 56.34          & 57.16          & 57.51          & 56.97          & 57.13          & 57.00          & 57.01          & 57.08          & 56.69          & 56.47          & 60.92             & \textbf{63.97} & 60.25             & 56.52            & 55.79             \\
Hate\textsubscript{David-17}      & 77.71        &     77.54                & 77.15                              & 77.47         & \textbf{78.28} & 76.87          & 77.46          & 77.55          & 77.22          & 78.13          & 78.26          & 78.16          & 77.93          & 76.45          & 77.00             & 77.29          & 76.93             & 77.07            & 77.13             \\
Humor\textsubscript{Potash-17}    & 54.40          &     54.80                   & 52.77                              & 55.45         & 55.26          & 55.32          & 52.49          & 50.06          & 54.60          & \textbf{57.14} & 55.10          & 55.25          & 55.57          & 54.75          & 54.93             & 55.51          & 53.83             & 53.33            & 50.07             \\
Humor\textsubscript{Meaney-21}    & 92.37     &      93.50                  & 94.46                              & 93.24         & 93.69          & 93.58          & 93.48          & 92.85          & \textbf{94.52} & 93.55          & 94.50          & 93.19          & 92.69          & 93.82          & 93.68             & 93.74          & 94.49             & 91.46            & 92.51             \\
Irony\textsubscript{Hee-18A}      & 73.93    &       74.46                   & 77.35                              & 74.52         & 74.97          & 74.50          & 75.16          & 73.97          & 76.24          & 75.34          & 77.93          & 74.40          & 75.62          & 76.63          & 72.73             & 76.22          & \textbf{79.89}    & 77.57            & 78.64             \\
Irony\textsubscript{Hee-18B}      & 52.30       &      50.70                    & 58.67                              & 52.91         & 53.79          & 51.43          & 49.29          & 50.41          & 54.76          & 54.94          & 56.09          & 54.73          & 52.47          & 57.59          & 56.11             & 60.14          & \textbf{61.67}    & 54.37            & 55.20             \\
Offense\textsubscript{-Zamp-19}   & 80.13     &     80.38                   & 78.49                              & 79.97         & 80.24          & 79.74          & 79.34          & 79.95          & 78.87          & 80.18          & 81.14          & 80.18          & 80.65          & 80.18          & \textbf{81.34}    & 79.82          & 79.50             & 79.65            & 79.26             \\
Sarc\textsubscript{Riloff-13}     & 73.85        &      73.90                  & 78.81                              & 72.02         & 75.24          & 71.42          & 74.72          & 74.16          & 75.88          & 76.52          & 77.93          & 76.30          & 80.10          & 78.34          & 78.74             & \textbf{80.50} & 80.49             & 77.41            & 78.09             \\
Sarc\textsubscript{Ptacek-14}     & 95.09          &      96.15             & \textbf{96.35}                     & 95.81         & 95.64          & 95.50          & 95.62          & 95.24          & 95.81          & 95.81          & 96.06          & 95.67          & 96.01          & 95.88          & 96.16             & 96.01          & 96.24             & 95.72            & 96.26             \\
Sarc\textsubscript{Rajad-15}      & 85.07    &    85.63                     & 87.58                              & 86.18         & 86.23          & 85.04          & 85.55          & 85.20          & 85.93          & 86.14          & 86.65          & 86.02          & 86.94          & 86.80          & 87.48             & 87.56          & \textbf{88.92}    & 85.99            & 88.10             \\
Sarc\textsubscript{Bam-15}        & 79.08   &    79.27                      & 82.08                              & 80.03         & 80.13          & 80.22          & 80.16          & 79.83          & 80.31          & 80.73          & 81.12          & 81.13          & 81.73          & 81.48          & 82.53             & 81.19          & 81.53             & 80.70            & \textbf{82.64}    \\
Senti\textsubscript{Rosen-17}     & 71.08           &      71.55            & 71.83                              & 72.03         & \textbf{72.65} & 72.10          & 71.99          & 71.84          & 71.82          & 72.24          & 71.98          & 72.27          & 71.56          & 71.27          & 72.07             & 71.83          & 71.08             & 70.66            & 69.48             \\
Stance\textsubscript{Moham-16}    & 70.41          &      67.00             & 67.41                              & 67.14         & 69.94          & 69.51          & 68.13          & 69.23          & 69.68          & 70.20          & 68.62          & 70.04          & 68.48          & 69.06          & 69.65             & \textbf{71.27} & 70.77             & 69.11            & 69.22             \\ \cdashline{1-20}
Average                                            & 75.78    &75.80                         & 77.10                              & 75.92         & 76.60          & 75.90          & 75.69          & 75.51          & 76.59          & 76.92          & 77.30          & 76.78          & 76.96          & 76.94          & 77.43             & 77.97          & \textbf{78.12}    & 76.08            & 76.26             \\ \bottomrule 


\end{tabular}
\caption{Summary performance of our models across different \textbf{(i)} PM and SFT settings, \textbf{(ii)} single and multi-task settings, and \textbf{(iii)} in comparison with the BERTweet~\cite{nguyen-etal-2020-bertweet}, a SOTA Twitter pre-trained language model. The metric is macro $F_1$.}\label{tab:full_res}
% \end{table}

\end{sidewaystable}

==> table/illustration.tex <==
\begin{figure*}[h]
\centering
\begin{subfigure}[]{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{latex/table/pragmatic_masking.png}
  \caption{Pragmatic masking}
  \label{fig:pm}
\end{subfigure}%
\begin{subfigure}[]{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{latex/table/sft.png}
  \caption{Surrogate fine-tuning}
  \label{fig:sft}
\end{subfigure}
\caption{Illustration of our proposed pragmatic masking and surrogate fine-tuning.}
\label{fig:illustration}
\end{figure*}


==> table/mt_res.tex <==
\begin{table}[]
\centering
\tiny 
\begin{tabular}{@{}lcc:ccc@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Task}}} & \multicolumn{2}{c}{\textbf{RoBERTa\textsubscript{BASE}}}                                   & \multicolumn{3}{c}{\textbf{Our Methods}}                                                                                \\  \cmidrule(lr){2-3} \cmidrule(lr){4-6} 
\multicolumn{1}{c}{}                               & \multicolumn{1}{c}{\textbf{SG}} & \multicolumn{1}{c}{\textbf{MT}} & \multicolumn{1}{c}{\textbf{SG\textsubscript{PM-EA}}} & \multicolumn{1}{c}{\textbf{SG\textsubscript{SFT-H}}} & \multicolumn{1}{c}{\textbf{SG\textsubscript{Best}}} \\ \midrule
Crisis\textsubscript{Oltea}       & 95.95                           & 95.88                           & \textbf{95.98}                         & 95.87                                  & 95.68                                 \\
Emo\textsubscript{Moham}          & 77.99                           & 75.79                           & \textbf{81.09}                         & 78.69                                  & 80.50                                 \\
Hate\textsubscript{Waseem}        & 57.34                           & 56.52                           & 57.01                                  & \textbf{63.97}                         & 60.25                                 \\
Hate\textsubscript{David}         & 77.71                           & 77.07                           & \textbf{78.26}                         & 77.29                                  & 76.93                                 \\
Humor\textsubscript{Potash}       & 54.40                           & 53.33                           & 55.10                                  & 55.51                                  & 53.83                                 \\
Humor\textsubscript{Meaney}       & 92.37                           & 91.46                           & \textbf{94.50}                         & 93.74                                  & 94.49                                 \\
Irony\textsubscript{Hee-A}        & 73.93                           & 77.57                           & 77.93                                  & 76.22                                  & \textbf{79.89}                        \\
Irony\textsubscript{Hee-B}        & 52.30                           & 54.37                           & 56.09                                  & 60.14                                  & \textbf{61.67}                        \\
Offense\textsubscript{Zamp}       & 80.13                           & 79.65                           & \textbf{81.14}                         & 79.82                                  & 79.50                                 \\
Sarc\textsubscript{Riloff}        & 73.85                           & 77.41                           & 77.93                                  & \textbf{80.50}                         & 80.49                                 \\
Sarc\textsubscript{Ptacek}        & 95.09                           & 95.72                           & 96.06                                  & 96.01                                  & \textbf{96.24}                        \\
Sarc\textsubscript{Rajad}         & 85.07                           & 85.99                           & 86.65                                  & 87.56                                  & \textbf{88.92}                        \\
Sarc\textsubscript{Bam}           & 79.08                           & 80.70                           & 81.12                                  & 81.19                                  & \textbf{81.53}                        \\
Senti\textsubscript{Rosen}        & 71.08                           & 70.66                           & \textbf{71.98}                         & 71.83                                  & 71.08                                 \\
Stance\textsubscript{Moham}       & 70.41                           & 69.11                           & 68.62                                  & \textbf{71.27}                         & 70.77                                 \\ \cdashline{1-6}
Average                                            & 75.78                           & 76.08                           & 77.30                                  & 77.97                                  & \textbf{78.12}                        \\ \bottomrule
\end{tabular}


\caption{Multi-task learning. \textbf{Bold front} indicates best result for each task. RoBERTa\textsubscript{BASE} is the baseline without further pre-training. \textbf{SFT:} Surrogate fine-tuning, \textbf{SG:} Single task, \textbf{MT:} Multi-task. \textbf{SG\textsubscript{PM-EA:}} Single task PM with emoji anywhere, \textbf{SG\textsubscript{SFT-H}:} Single task SFT with hashtags, \textbf{SG\textsubscript{Best}:} Single task PM with emoji anywhere surrogate fine-tuned on hashtags (setting X2-SFT-H in Table~\ref{tab:sft_res}, which is our best model).}\label{tab:mtl_res}
\end{table}


% \begin{table}[]
% \centering
% \footnotesize
% \begin{tabular}{@{}lrr|rr@{}}
% \toprule
% \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Task}}} & \multicolumn{2}{c}{\textbf{Baseline}}                                   & \multicolumn{2}{c}{\textbf{SFT}}                                \\ \cmidrule(l){2-5} 
% \multicolumn{1}{c}{}                               & \multicolumn{1}{c}{\textbf{SG-Base}} & \multicolumn{1}{c}{\textbf{MT-Base}} & \multicolumn{1}{c}{\textbf{SG-SFT}} & \multicolumn{1}{c}{\textbf{MT-SFT}} \\ \midrule
% Crisis\textsubscript{Oltea}       & 95.95                           & 95.93                           & 95.87                           & 95.84                           \\
% Emo\textsubscript{Moham}          & 77.99                           & 76.39                           & \colorbox{orange!10}{78.69}                     & 74.90                           \\
% Hate\textsubscript{Waseem}        & 57.34                           & 57.13                           & \colorbox{orange!10}{63.97}                     & 55.36                           \\
% Hate\textsubscript{David}         & 77.71                           & \colorbox{orange!10}{\textbf{77.82}}            & 77.29                           & 76.30                           \\
% Humor\textsubscript{Potash}       & 54.40                           & 53.78                           & \colorbox{orange!10}{55.51}                     & \colorbox{orange!10}{55.14}                     \\
% Humor\textsubscript{Meaney}       & 90.33                           & 89.43                           & \colorbox{orange!10}{92.02}                     & 89.77                           \\
% Irony\textsubscript{Hee-A}        & 73.93                           & \colorbox{orange!10}{\textbf{78.27}}            & \colorbox{orange!10}{76.22}                     & \colorbox{orange!10}{\textbf{78.35}}            \\
% Irony\textsubscript{Hee-B}        & 52.30                           & \colorbox{orange!10}{\textbf{53.17}}            & \colorbox{orange!10}{60.14}                     & \colorbox{orange!10}{54.21}                     \\
% Offense\textsubscript{Zamp}       & 80.13                           & 79.71                           & 79.82                           & 76.81                           \\
% Sarc\textsubscript{Riloff}        & 73.85                           & \colorbox{orange!10}{\textbf{81.10}}            & \colorbox{orange!10}{80.50}                     & \colorbox{orange!10}{\textbf{80.84}}            \\
% Sarc\textsubscript{Ptacek}        & 95.09                           & \colorbox{orange!10}{\textbf{95.98}}            & \colorbox{orange!10}{96.01}                     & \colorbox{orange!10}{\textbf{96.15}}            \\
% Sarc\textsubscript{Rajad}         & 85.07                           & \colorbox{orange!10}{\textbf{86.01}}            & \colorbox{orange!10}{87.56}                     & \colorbox{orange!10}{86.63}                     \\
% Sarc\textsubscript{Bam}           & 79.08                           & \colorbox{orange!10}{\textbf{80.69}}            & \colorbox{orange!10}{81.19}                     & \colorbox{orange!10}{\textbf{81.91}}            \\
% Senti\textsubscript{Rosen}        & 71.08                           & 71.04                           & 71.83                           & 69.77                           \\
% Stance\textsubscript{Moham}       & 70.41                           & 69.02                           & 71.27                           & 69.06                           \\ \cdashline{1-5} 
% \textbf{Average}                                   & 75.64                           & \colorbox{orange!10}{\textbf{76.36}}            & \colorbox{orange!10}{77.86}                     & \colorbox{orange!10}{76.07}                     \\ \bottomrule
% \end{tabular}
% \caption{Multi-task learning. Bold front indicate that the MT model outperform corresponding single task model. \textbf{Baseline}: RoBERTa\textsubscript{BASE} without further pre-training, \textbf{SFT}: surrogate fine-tuning, \textbf{SG}: single task, \textbf{MT}: multi-task.}\label{tab:mtl_res}
% \end{table}

==> table/para_data.tex <==
\subsection{SMPB}
We fine-tune the paraphrase model on the Train split of each of our $15$ datasets, using top-$p$~\cite{holtzman2019curious} with $p=0.95$ to generate $10$ paraphrases for each gold sample. To remove any `paraphrases' that are just copies of the original tweet or near-duplicates, we use a simple tri-gram similarity method. That is, we remove any sequences whose similarity with the original tweet is $> 0.95$. We also remove paraphrases of the same tweet that are $> 50\%$ similar to one another. To ensure that paraphrases are not very different from the original tweets, we also remove any sequences whose similarity with original tweets $=0$. This process results in a paraphrasing dataset \texttt{Para-Clean}. Table~\ref{tab:append_para} shows the distribution of the resulting paraphrase datasets.  %Table~\ref{tab:para_exam_app} provides more paraphrase examples. 

\input{table/para_data_table}
\vspace{-5pt}
We present an example paraphrase in Figure~\ref{fig:para}. We observe that the paraphrase model fails to generate emojis since emojis are out-of-vocabulary for the T5 model, but the model can preserve the overall semantics of the original tweet.
%~~~~~~~~~~~~~~~~~~~~~~~~
\begin{figure}[h]
\begin{centering}
 \includegraphics[scale=0.26]{emojis/example_para.PNG}\vspace{-7pt}
  \caption{Paraphrase example.} \vspace{-10pt}
  \label{fig:para}
\end{centering}
\end{figure}
%~~~~~~~~~~~~~~~~~~~~~~~~




% \begin{table}[h]
% \centering
% \footnotesize
% \begin{tabular}{@{}lrrrr@{}}
% \toprule
% \multicolumn{1}{c}{\textbf{Task}}                & \multicolumn{1}{c}{\textbf{Para1}} & \multicolumn{1}{c}{\textbf{Para2}} & \multicolumn{1}{c}{\textbf{Para4}} & \multicolumn{1}{c}{\textbf{Para5}} \\ \midrule
% Crisis\textsubscript{Oltea}  & 48,065                             & 86,765                             & 120,731                            & 123,879                            \\
% Emo\textsubscript{Moham}     & 3,257                              & 6,288                              & 10,886                             & 12,227                             \\
% Hate\textsubscript{Waseem}   & 8,683                              & 16,570                             & 28,323                             & 31,698                             \\
% Hate\textsubscript{David}    & 19,826                             & 38,177                             & 65,481                             & 73,367                             \\
% Humor\textsubscript{Potash}  & 11,325                             & 21,820                             & 38,318                             & 43,952                             \\
% Humor\textsubscript{Meaney}  & 7,200                              & 14,152                             & 25,741                             & 29,601                             \\
% Irony\textsubscript{Hee-A}    & 3,450                              & 6,646                              & 11,413                             & 12,777                             \\
% Irony\textsubscript{Hee-B}    & 3,450                              & 6,639                              & 11,469                             & 12,850                             \\
% Offense\textsubscript{Zamp} & 11,916                             & 22,951                             & 39,583                             & 44,348                             \\
% Sarc\textsubscript{Riloff}   & 1,413                              & 2,713                              & 4,628                              & 5,167                              \\
% Sarc\textsubscript{Ptacek}   & 71,433                             & 138,870                            & 242,065                            & 272,362                            \\
% Sarc\textsubscript{Rajad}    & 41,261                             & 78,328                             & 131,533                            & 146,605                            \\
% Sarc\textsubscript{Bam}      & 11,864                             & 22,434                             & 37,475                             & 41,570                             \\
% Senti\textsubscript{Rosen}   & 42,756                             & 84,299                             & 154,378                            & 178,147                            \\
% Stance\textsubscript{Moham}  & 2,622                              & 4,717                              & 6,425                              & 6,609                              \\ \bottomrule
% \end{tabular} 
% \caption{Distribution of SMPB Train set.}\label{tab:paraphrase}
% \end{table}

==> table/para_data_table.tex <==
\begin{table}[h]
\centering
\tiny
\resizebox{0.85\columnwidth}{!}{%
\begin{tabular}{@{}lrrrr@{}}
\toprule
\multicolumn{1}{c}{\textbf{Task}}                & \multicolumn{1}{c}{\textbf{Para1}} & \multicolumn{1}{c}{\textbf{Para2}} & \multicolumn{1}{c}{\textbf{Para4}} & \multicolumn{1}{c}{\textbf{Para5}} \\ \midrule
Crisis\textsubscript{Oltea}  & $48.1$K                             & $86.8$K                             & $120.7$K                           & $123.9$K                         \\
Emo\textsubscript{Moham}     & $3.3$K                              & $6.3$K                             & $10.9$K                           & $12.2$K                          \\
Hate\textsubscript{Waseem}   & $8.7$K                             & $16.6$K                           & $28.3$K                          & $31.7$K                          \\
Hate\textsubscript{David}    & $19.8$K                          & $38.2$K                          & $65.5$K                          & $73.4$K                           \\
Humor\textsubscript{Potash}  & $11.3$K                         & $21.8$K                            & $38.3$K                          & $44.0$K                             \\
Humor\textsubscript{Meaney}  & $8.0$K                            & $15.7$K                            & $28.7$K                        & $33.0$K                          \\
Irony\textsubscript{Hee-A}    & $3.5$K                          & $6.6$K                             & $11.4$K                           & $12.8$K                            \\
Irony\textsubscript{Hee-B}    & $3.5$K                            & $6.6$K                            & $11.5$K                           & $12.9$K                           \\
Offense\textsubscript{Zamp} & $11.9$K                            & $23.0$K                             & $39.6$K                           & $44.3$K                           \\
Sarc\textsubscript{Riloff}   & $1.4$K                            & $2.7$K                             & $4.6$K                            & $5.2$K                           \\
Sarc\textsubscript{Ptacek}   & $71.4$K                     & $138.9$K                            & $242$K                          & $272.4$K                          \\
Sarc\textsubscript{Rajad}    & $41.3$K                             & $78.3$K                           & $131.5$K                           & $146.6$K                          \\
Sarc\textsubscript{Bam}      & $11.9$K                          & $22.4$K                           & $37.5$K                           & $41.6$K                           \\
Senti\textsubscript{Rosen}   & $42.8$K                          & $84.3$K                           & $154.8$K                          & $178.1$K                        \\
Stance\textsubscript{Moham}  & $2.6$K                             & $4.7$K                             & $6.4$K                            & $6.6$K                              \\ \bottomrule
\end{tabular}%
} \vspace{-5pt}
\caption{Distribution of SMPB Train set.}\label{tab:append_para}
\end{table}

==> table/para_res.tex <==
\begin{table*}[]
\scriptsize
\centering
\begin{tabular}{@{}lcccc:cc|cccc:cc@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Task}}} & \multicolumn{6}{c}{\textbf{Baseline (RoBERTa\textsubscript{BASE})}}                                            & \multicolumn{6}{c}{\textbf{Our Best Method (X2+SFT-H)}}                                              \\ \cmidrule(lr){2-7} \cmidrule(lr){8-13} 
\multicolumn{1}{c}{}                               & \textbf{P1} & \textbf{P2} & \textbf{P4} & \textbf{P5} & \textbf{Best} & \textbf{Gold} & \textbf{P1} & \textbf{P2} & \textbf{P4} & \textbf{P5} & \textbf{Best} & \textbf{Gold} \\ \midrule
Crisis\textsubscript{Oltea}       & \textbf{95.54}       & 95.20       & 95.23       & 95.39       & 95.54         & 95.95         & 94.98       & 94.68       & 95.05       & \textbf{95.09}       & 95.09         & 95.68         \\
Emo\textsubscript{Moham}          & 77.06       & \textbf{77.43}       & 77.31       & 76.99       & 77.43         & 77.99         & 77.81       & \textbf{78.38}       & 77.61       & 77.84       & 78.38         & 80.50         \\
Hate\textsubscript{Waseem}        & 54.58       & \textbf{54.92}       & 54.83       & 54.63       & 54.92         & 57.34         & 53.48       & \textbf{54.39}       & 53.94       & 54.11       & 54.39         & 60.25         \\
Hate\textsubscript{David}         & 74.04       & 75.26       & \textbf{75.80}       & 74.97       & 75.80         & 77.71         & 73.12       & 74.48       & 74.08       & \textbf{74.66}       & 74.66         & 76.93         \\
Humor\textsubscript{Potash}       & 49.26       & 53.16       & \textbf{53.54}       & 53.34       & 53.54         & 54.40         & 49.61       & \textbf{54.39}       & 52.59       & 51.90       & 54.39         & 53.83         \\
Humor\textsubscript{Meaney}       & 91.71       & 91.66       & \textbf{92.28}       & 91.77       & 92.28         & 92.37         & 94.13       & \textbf{94.32}       & 93.95       & 94.16       & 94.32         & 94.49         \\
Irony\textsubscript{Hee-A}        & 71.00       & \textbf{71.53}       & 71.06       & 71.53       & 71.53         & 73.93         & 74.41       & 75.53       & 75.40       & \textbf{75.67}       & 75.67         & 79.89         \\
Irony\textsubscript{Hee-B}        & 43.24       & 45.69       & 48.02       & \textbf{48.33}       & 48.33         & 52.30         & 48.88       & \textbf{51.71}       & 50.56       & 49.69       & 51.71         & 61.67         \\
Offense\textsubscript{Zamp}       & 79.90       & 79.95       & \textbf{80.15}       & 79.57       & 80.15         & 80.13         & 75.96       & 78.22       & 78.23       & \textbf{78.80}       & 78.80         & 79.50         \\
Sarc\textsubscript{Riloff}        & 71.40       & \textbf{72.74}       & 72.45       & 72.26       & 72.74         & 73.85         & 76.91       & 77.59       & \textbf{79.41}       & 79.24       & 79.41         & 80.49         \\
Sarc\textsubscript{Ptacek}        & 90.54       & 92.58       & \textbf{93.70}       & 93.62       & 93.70        & 95.09         & 91.65       & 93.31       & \textbf{94.10}       & 93.98       & 94.10         & 96.24         \\
Sarc\textsubscript{Rajad}         & 81.00       & 81.94       & 82.53       & \textbf{82.64}       & 82.64         & 85.07         & 87.34       & 86.88       & \textbf{87.59}       & 87.38       & 87.59         & 88.92         \\
Sarc\textsubscript{Bam}           & 77.60       & 76.93       & \textbf{77.92}       & 77.76       & 77.92         & 79.08         & 80.86       & 80.06       & \textbf{81.53}       & 80.22       & 81.53         & 81.53         \\
Senti\textsubscript{Rosen}        & 70.50       & 70.95       & 71.51       & \textbf{71.52}       & 71.52         & 71.08         & 66.79       & 67.31       & \textbf{68.87}       & 68.29       & 68.87         & 71.08         \\
Stance\textsubscript{Moham}       & 67.75       & 69.07       & \textbf{69.30}       & 67.34       & 69.30         & 70.41         & 68.39       & \textbf{68.60}       & 68.58       & 67.03       & 68.60         & 70.77         \\ \cdashline{1-13} 
Average                                            & 73.01       & 73.93       & \textbf{74.38}       & 74.11       & \textbf{74.49}         & 75.78         & 74.29       & 75.32       & \textbf{75.43}       & 75.20       & \textbf{75.83}         & 78.12         \\ \bottomrule
\end{tabular} %\vspace{-5pt}
\caption{Results of paraphrasing-based model. \textbf{Gold} denotes a model fine-tuned with downstream, original Train data. \textbf{P$n$} indicates that the model is trained on Para$n$ training set. \textbf{Bold} denotes the best paraphrase result for each task within each of two settings (Baseline vs. X2+SFT-H). X2+SFT-H: Our model combining best settings of PM and SFT (see Table~\ref{tab:sft_res}). \textbf{Best}: Performance of the best paraphrasing setting. An ensemble of our best paraphrase-based models is slightly better than the gold-initialized baseline model. \vspace{-10pt}}~\label{tab:para_res} 
\end{table*}



% \begin{table*}[t]
% \scriptsize
% \centering
% \begin{tabular}{@{}lcccc:cccccc:cc@{}}
% \toprule
% \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Task}}} & \multicolumn{6}{c}{\textbf{Baseline (RoBERTa\textsubscript{BASE})}}                                                                                        & \multicolumn{6}{c}{\textbf{Surrogate Fine-tuning (SFT)}}                                                                           \\ \cmidrule(l){2-13} 
% \multicolumn{1}{c}{}                               & \textbf{P1}                     & \textbf{P2}                     & \textbf{P4}                     & \textbf{P5}                     & \textbf{P-Best} & \multicolumn{1}{c|}{\textbf{Gold}} & \textbf{P1} & \textbf{P2}                     & \textbf{P4}                     & \textbf{P5}                     & \textbf{P-Best} & \textbf{Gold} \\ \midrule
% Crisis\textsubscript{Oltea}       & \textbf{95.54} & 95.20                           & 95.23                           & 95.39                           & 95.54           & \multicolumn{1}{c|}{95.95}         & 95.07       & 94.99                           & \textbf{95.12} & 95.06                           & 95.12           & 95.87         \\
% Emo\textsubscript{Moham}          & 77.06                           & \textbf{77.43} & 77.31                           & 76.99                           & 77.43           & \multicolumn{1}{c|}{77.99}         & 75.85       & \textbf{76.94} & 76.45                           & 76.63                           & 76.94           & 78.69         \\
% Hate\textsubscript{Waseem}        & 54.58                           & \textbf{54.92} & 54.83                           & 54.63                           & 54.92           & \multicolumn{1}{c|}{57.34}         & 54.01       & \textbf{54.89} & 54.65                           & 54.52                           & 54.89           & 63.97         \\
% Hate\textsubscript{David}         & 74.04                           & 75.26                           & \textbf{75.80} & 74.97                           & 75.80           & \multicolumn{1}{c|}{77.71}         & 72.54       & 74.06                           & 73.71                           & \textbf{75.27} & 75.27           & 77.29         \\
% Humor\textsubscript{Potash}       & 49.26                           & 53.16                           & \textbf{53.54} & 53.34                           & 53.54           & \multicolumn{1}{c|}{54.40}         & 50.38       & 51.99                           & 51.62                           & \textbf{53.22} & 53.22           & 55.51         \\
% Humor\textsubscript{Meaney}       & 88.67                           & 88.85                           & \textbf{89.11} & 88.16                           & 89.11           & \multicolumn{1}{c|}{90.33}         & 90.33       & 89.73                           & \textbf{90.46} & 89.21                           & 90.46           & 92.02         \\
% Irony\textsubscript{Hee-A}        & 71.00                           & 71.53                           & 71.06                           & \textbf{71.53} & 71.53           & \multicolumn{1}{c|}{73.93}         & 72.89       & 73.43                           & \textbf{75.28} & 74.29                           & 75.28           & 76.22         \\
% Irony\textsubscript{Hee-B}        & 43.24                           & 45.69                           & 48.02                           & \textbf{48.33} & 48.33           & \multicolumn{1}{c|}{52.30}         & 49.01       & 49.08                           & \textbf{51.82} & 51.14                           & 51.82           & 60.14         \\
% Offense\textsubscript{Zamp}       & 79.90                           & 79.95                           & \textbf{80.15} & 79.57                           & 80.15           & \multicolumn{1}{c|}{80.13}         & 77.98       & \textbf{79.41} & 78.96                           & 79.10                           & 79.41           & 79.82         \\
% Sarc\textsubscript{Riloff}        & 71.40                           & \textbf{72.74} & 72.45                           & 72.26                           & 72.74           & \multicolumn{1}{c|}{73.85}         & 74.27       & 76.86                           & 77.26                           & \textbf{78.36} & 78.36           & 80.50         \\
% Sarc\textsubscript{Ptacek}        & 90.54                           & 92.58                           & \textbf{93.70} & 93.62                           & 93.70           & \multicolumn{1}{c|}{95.09}         & 90.85       & 92.69                           & 93.57                           & \textbf{93.61} & 93.61           & 96.01         \\
% Sarc\textsubscript{Rajad}         & 81.00                           & 81.94                           & 82.53                           & \textbf{82.64} & 82.64           & \multicolumn{1}{c|}{85.07}         & 85.71       & 86.13                           & 86.19                           & \textbf{86.32} & 86.32           & 87.56         \\
% Sarc\textsubscript{Bam}           & 77.60                           & 76.93                           & \textbf{77.92} & 77.76                           & 77.92           & \multicolumn{1}{c|}{79.08}         & 80.20       & 80.05                           & \textbf{80.90} & 80.22                           & 80.90           & 81.19         \\
% Senti\textsubscript{Rosen}        & 70.50                           & 70.95                           & 71.51                           & \textbf{71.52} & 71.52           & \multicolumn{1}{c|}{71.08}         & 67.35       & 68.20                           & \textbf{69.18} & 68.59                           & 69.18           & 71.83         \\
% Stance\textsubscript{Moham}       & 67.75                           & 69.07                           & \textbf{69.30} & 67.34                           & 69.30           & \multicolumn{1}{c|}{70.41}         & 67.61       & \textbf{69.61} & 68.20                           & 69.47                           & 69.61           & 71.27         \\ \cdashline{1-13} 
% \textbf{Average}                  & 72.81                           & 73.75                           & 74.17                           & 73.87                           & 74.28           & \multicolumn{1}{c|}{75.64}         & 73.60       & 74.54                           & 74.89                           & 75.00                           & 75.36           & 77.86         \\ \bottomrule
% \end{tabular} \vspace{-5pt}
% \caption{Results of paraphrasing-based model. \textbf{Gold} denotes the model train with original Train dataset. \textbf{P$n$} indicates that the model is trained on Para$n$ training set. \textbf{Bold font} denotes the best paraphrase result for each task within each of two settings (Baseline vs. SFT). \textbf{P-Best} is the performance of the best paraphrasing setting. \vspace{-10pt}}~\label{tab:para_res} 
% \end{table*}

==> table/para_sample.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\centering
\tiny
\begin{tabular}{@{}ll@{}}
\toprule
\textbf{Orignial Tweet}              & \begin{tabular}[c]{@{}l@{}}Being stuck in the roof of your house provides amazing view but sheer terror \\ of falling down, kinda like life\end{tabular}                                                                   \\ \midrule
\multirow{5}{*}{\textbf{Paraphrase}} & \begin{tabular}[c]{@{}l@{}}Life When I Get In the Roof of My House Provides a View But Terror of Falling Down, \\ You hate being stuck in your roof. This is what makes me want to fall, for lack of room.\end{tabular}    \\
                                     & \begin{tabular}[c]{@{}l@{}}Life When I Get In the Roof of My House Provides a View But Terror of Falling \\ Down, You hate being stuck in your roof. This is what makes me want to fall, \\ for lack of room.\end{tabular} \\
                                     & \begin{tabular}[c]{@{}l@{}}Beyond and up! Finding yourself in the roof gives you amazing views but sheer \\ terror of falling...\end{tabular}                                                                              \\
                                     & \begin{tabular}[c]{@{}l@{}}Imagine being stuck in the roof of your house providing amazing view but sheer \\ terror of falling down. Life is hard.\end{tabular}                                                            \\
                                     & From the roof of your house, you have a great view but you're scared of falling down                                                                                                                                       \\ \bottomrule
\end{tabular}
\end{table}

==> table/para_sample_app.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[h!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{llc}
\toprule
\textbf{Original Tweet}                                                                                                                                                & \textbf{Paraphrase}                                                                                   & \textbf{Label}                                 \\ \toprule
                                                                                                                                                                       & You guys are horrible, avoid MMT                                                                       & { }                        \\
                                                                                                                                                                       & what I am doing is in my control, \#AvoidMMT, you guys are terrifying                                  & { }                        \\ 
                                                                                                                                                                       & You guys are \#terrorist. I have used everything I have to do.                                         & { }                        \\
\multirow{-4}{*}{\begin{tabular}[c]{@{}l@{}}USER but what I am doing is in my control, \\ \#AvoidMMT , you guys are \#terrible\end{tabular}}                           & You guys are awful, but I am going to stop doing it.                                                   & \multirow{-4}{*}{{ anger}} \\\hline
                                                                                                                                                                       & I hate when people say 'I need to talk to you or we need to talk to you'. I guess that's the problem.  &                                                \\
                                                                                                                                                                       & I hate when people tell me 'I need to talk to you or we need to speak' my anxiety immediately goes up. &                                                \\
\multirow{-3}{*}{\begin{tabular}[c]{@{}l@{}}I hate when people say 'I need to talk to you or we need to talk.' \\ My anxiety immediately goes up...\end{tabular}}      & Why am I afraid when people say 'I need to talk to you or we need to talk?'                            & \multirow{-3}{*}{anger}                        \\\hline
                                                                                                                                                                       & The 46th wedding I've ruined. When I hit 50 I can retire. It's nice to see yo                          &                                                \\
                                                                                                                                                                       & Here's the 47th wedding I've ruined. If I'm old enough to go on the 40s I can get married.             &                                                \\
\multirow{-3}{*}{This is the 47th wedding I've ruined. When I hit 50 I can retire.}                                                                                    & After a single wedding, I drew 47 weddings, and before I hit 50 I can retire"                          & \multirow{-3}{*}{humor}                        \\\hline
                                                                                                                                                                       & Sorry to disturb you. I have absolutely no idea what time I'll be on cam tomorrow.                     &                                                \\
\multirow{-2}{*}{\begin{tabular}[c]{@{}l@{}}Sorry guys I have absolutely no idea \\ what time i'll be on cam tomorrow but will keep you posted.\end{tabular}}          & I have absolutely no idea what time I'll be on camera tomorrow but I'll keep you posted                & \multirow{-2}{*}{sadness}                      \\\hline
                                                                                                                                                                       & "I'll buy you Dunkin' Donuts for \$5.                                                                  &                                                \\
                                                                                                                                                                       & Who wants to go with me for my tattoo tomorrow? I'll buy you a Dunkin' Donuts.                         &                                                \\
\multirow{-3}{*}{\begin{tabular}[c]{@{}l@{}}Who wants to go with me to get my tattoo tomorrow? \\ I'll buy you Dunkin doughnuts\end{tabular}}                          & Who wants to go with me to get my tattoo tomorrow?                                                     & \multirow{-3}{*}{neutral}                      \\\hline
                                                                                                                                                                       & The day before class please eat beans, onions and garlic. Also see the videos                          &                                                \\
                                                                                                                                                                       & "The Day Before Class. You should make that meal, (do you think).                                      &                                                \\
\multirow{-3}{*}{\begin{tabular}[c]{@{}l@{}}USER May I suggest, that you have a meal that is made with \\ beans, onions \& garlic, the day before class.\end{tabular}} & If you can eat just the day before class, make a wonderful meal with garlic, onions and beans.         & \multirow{-3}{*}{joy} \\                        
        \toprule               
\end{tabular}%
}
\caption{Examples of paraphrases in SMPB}
\label{tab:para_exam_app}
\end{table*}
